Revisiting Quantum Algorithms for Linear Regressions: Quadratic Speedups without Data-Dependent Parameters

Linear regression is one of the most fundamental linear algebra problems. Given a dense matrix $A \in \mathbb{R}^{n \times d}$ and a vector $b$, the goal is to find $x'$ such that $ \| Ax' - b \|_2^2 \leq (1+\epsilon) \min_{x} \| A x - b \|_2^2 $. The best classical algorithm takes $O(nd) + \mathrm{poly}(d/\epsilon)$ time [Clarkson and Woodruff STOC 2013, Nelson and Nguyen FOCS 2013]. On the other hand, quantum linear regression algorithms can achieve exponential quantum speedups, as shown in [Wang Phys. Rev. A 96, 012335, Kerenidis and Prakash ITCS 2017, Chakraborty, Gily{\'e}n and Jeffery ICALP 2019]. However, the running times of these algorithms depend on some quantum linear algebra-related parameters, such as $\kappa(A)$, the condition number of $A$. In this work, we develop a quantum algorithm that runs in $\widetilde{O}(\epsilon^{-1}\sqrt{n}d^{1.5}) + \mathrm{poly}(d/\epsilon)$ time. It provides a quadratic quantum speedup in $n$ over the classical lower bound without any dependence on data-dependent parameters. In addition, we also show our result can be generalized to multiple regression and ridge linear regression.

==> related.tex <==
\section{Related Work}


\label{sec:related_work}

\paragraph{Quantum optimization algorithms}

Quantum optimization algorithms have emerged as a promising approach to solving complex combinatorial optimization problems. These algorithms harness principles from quantum mechanics, such as superposition \cite{gaw19} and entanglement \cite{czm+22}, to efficiently explore vast search spaces. Quantum annealing, rooted in adiabatic quantum computation, involves encoding an optimization problem into the Hamiltonian of a quantum system \cite{snk12}. As the system evolves, it concurrently explores multiple configurations, ultimately settling into the ground state of the problem Hamiltonian, representing the optimal solution \cite{kn98,fggs00}.

The quantum approximate optimization algorithm (QAOA) is a hybrid quantum-classical approach employing a shallow quantum circuit to sample from a probability distribution of potential solutions \cite{ejs14}. Additionally, the quantum alternating operator ansatz utilizes a parameterized quantum circuit with alternating unitary operators to sample solutions for combinatorial optimizations \cite{hwo+19}.

The variational quantum eigensolver (VQE) is a hybrid algorithm utilizing a parameterized quantum circuit to prepare trial states \cite{pms14}. The classical optimizer updates the circuit parameters based on the measured expectation value of the problem Hamiltonian. The resulting optimized state approximates the ground state of the problem Hamiltonian. VQE has found applications in small molecule simulations and various optimization problems.




Moreover, linear programming and semidefinite programming are fundamental problems in the field of optimization. Recently, there has been a long list of work trying to give a fast quantum linear programming and semidefinite programming solvers
\cite{bs17,aggw17,bkllsw19,ag18,kp20,hjs+22_quantum}. Other than that, there are also works about solving linear systems \cite{hhl08}, and estimating volumes of convex bodies \cite{cch+19}. Another big class of quantum algorithms for solving optimization problems includes the variational quantum algorithm \cite{csrs20}, variational quantum eigensolver \cite{pms14}, nash equilibria of quantum zero-sum games \cite{vvm+23}, QAOA \cite{ejs14}, estimation of unitary channels \cite{hko+23}, quantum Hamiltonians \cite{hkt22,blmt23}, and quantum neural network \cite{beer2020training}. Although these algorithms are likely to be implemented in noisy intermediate-scale quantum (NISQ) devices, their performances cannot be rigorously proved.



\paragraph{Quantum machine learning}

Quantum machine learning (QML) is an emerging field that explores how quantum computing can advance machine learning. Several quantum algorithms have been proposed to provide speedups or enhanced capabilities compared to their classical machine learning counterparts. One approach is the development of quantum versions of neural networks, which were first conceptualized in \cite{k95}. Recently, several implementations have been proposed using parameterizable quantum circuits as the neural network structure \cite{fn18,mnkf18}. Hybrid quantum-classical training strategies have been developed, employing techniques like parameter shift rules and gradient estimation methods. Moreover, quantum enhancements for specific neural network components have been proposed, such as quantum perceptrons leveraging quantum interference for faster convergence compared to classical perceptrons \cite{wdk+17}, and quantum convolutional neural networks based on quantum circuit architectures showing exponential advantages over classical networks for certain learning tasks \cite{ccl19}.

Beyond neural networks, some QML approaches formulate the learning problem within a kernel-based framework \cite{md19,bgv+20}. Quantum versions of cluster analysis \cite{lmr13}, principal component analysis \cite{rml14,lmr14_pca,t21}, and Bayesian networks \cite{lyc14,mw18} have been theorized to demonstrate quantum advantages under certain conditions. Ongoing research focuses on developing practical, scalable implementations of these algorithms.

Another promising QML technique is quantum sampling, using parameterized quantum circuits to generate samples from probability distributions \cite{hbm+21}. Quantum sampling approaches have been proposed for various applications such as generative modeling \cite{bgp+19,wsk+21}, anomaly detection \cite{clw+22}, and recommendation systems \cite{kp16,t19}.


More specifically, QML algorithms have been developed for a wide array of tasks, such as clustering \cite{h20,dlt23}, boosting \cite{am20}, support vector machine \cite{rml14}, principal component analysis \cite{lmr14_pca}, statistical query learning \cite{agy20}. Since the beautiful result of the quantum-inspired algorithm for the recommend system due to Tang \cite{t19}, there is a long list of Quantum inspired algorithms, e.g., principal component analysis \cite{t18}, low rank approximation \cite{glt18,cgt+20}, linear regression \cite{gst20}, singular value transformation \cite{bt23,tt23,t23}.

\paragraph{Classical Linear Algebra}

Given such a family $\Pi$, it is natural to apply an $S$ to $A$ and then solve the smaller problem directly. This is the so-called \emph{sketch-and-solve} paradigm. Sketch-and-solve has led to the development of fast algorithms for many problems, such as linear regression \cite{cw13,nn13}, low rank approximation with Frobenious norm \cite{cw13,nn13}, fairness of regression \cite{svwz23}, matrix CUR decomposition \cite{bw14,swz17,swz19}, weighted low rank approximation \cite{rsw16,syyz23}, entrywise $\ell_1$ norm low rank approximation \cite{swz17,swz19_neurips_l1}, tensor regression \cite{swyz21,rsz22,dssw18,djs+19,dsy23}, tensor low rank approximation \cite{swz19}, general norm column subset selection \cite{swz19_neurips_general}, low rank matrix completion \cite{gsyz23}, designing an efficient neural network training method \cite{qsy23}, and attention regression problem \cite{syz23,gswy23}.  

Sketching can also be adapted to an iterative process to reduce the cost of iteration. This is the so-called \emph{Iterate-and-sketch} approach and it has led to fast algorithms for many fundamental problems, such as linear programming \cite{cls19,sy21,jswz21,lsz+23}, empirical risk minimization \cite{lsz19,qszz23}, dynamic kernel estimation \cite{qrs+22}, projection maintenance \cite{syyz23_dp} semi-definite programming \cite{gs22}, John Ellipsoid computation \cite{syyz22}, Frank-Wolfe algorithm \cite{xss21,sxyz22}, reinforcement learning \cite{ssx23}, rational database \cite{qjs+22}, matrix sensing \cite{qsz23}, softmax-inspired regression \cite{dls23_softmax,gsy23_hyper,lsz23,ssz23}, submodular maximization \cite{qsw23}, federated learning \cite{swyz23,bsy23,gsy23}, discrepancy problem \cite{dsw22,sxz22}, non-convex optimization \cite{syz21,szz21,als+22,z22}.
